$n$-Reference Transfer Learning for Saliency Prediction

Benefiting from deep learning research and large-scale datasets, saliency prediction has achieved significant success in the past decade. However, it still remains challenging to predict saliency maps on images in new domains that lack sufficient data for data-hungry models. To solve this problem, we propose a few-shot transfer learning paradigm for saliency prediction, which enables efficient transfer of knowledge learned from the existing large-scale saliency datasets to a target domain with limited labeled examples. Specifically, very few target domain examples are used as the reference to train a model with a source domain dataset such that the training process can converge to a local minimum in favor of the target domain. Then, the learned model is further fine-tuned with the reference. The proposed framework is gradient-based and model-agnostic. We conduct comprehensive experiments and ablation study on various source domain and target domain pairs. The results show that the proposed framework achieves a significant performance improvement. The code is publicly available at \url{https://github.com/luoyan407/n-reference}.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> sec/abs.tex <==
\begin{abstract}

Benefiting from deep learning research and large-scale datasets, saliency prediction has achieved significant success in the past decade. 
However, it still remains challenging to predict saliency maps on images in new domains that lack sufficient data for data-hungry models. 
To solve this problem, we propose a few-shot transfer learning paradigm for saliency prediction, 
which enables efficient transfer of knowledge learned from the existing large-scale saliency datasets to a target domain with limited labeled examples. 
%It does not require any architecture changes to work with state-of-the-art saliency models. 
%The proposed referenced transfer learning is gradient-based, based upon the widely-used transfer learning scheme, \ie first training and then fine-tuning,
Specifically, 
very few target domain examples are used as the {\it reference} to train a model with a source domain dataset such that the training process can converge to a local minimum in favor of the target domain. 
Then, the learned model 
% from the training process 
is further fine-tuned with the {\it reference}.
The proposed framework is gradient-based and model-agnostic.
We conduct comprehensive experiments and ablation study on various source domain and target domain pairs. 
The results show that the proposed framework achieves a significant performance improvement. 
The code is publicly available at
\url{https://github.com/luoyan407/n-reference}.
% \url{https://anonymous.4open.science/r/569febd6-df65-4688-aedc-04cc046b7ad1/}.

\keywords{Deep learning, transfer learning, n-shot learning, reference process, saliency prediction}

%TL;DR: We introduce a few-shot transfer learning framework for saliency prediction, which is able to use very few samples from target domain to adapt the knowledge learned from the source domain to the target domain.

%The general idea of transfer learning is to use knowledge learned from tasks for which a lot of labelled data is available in settings where only little labelled data is available. Creating labelled data is expensive, so optimally leveraging existing datasets is key.

%Due to the prohibitive process of collecting human attention data, it is important to adapt knowledge in the existing saliency prediction datasets to a new domain that could be short of training samples and very different from the existing stimulus in terms of scene context. 
%In this work, we study how to adaptively transfer knowledge in the existing datasets to improve saliency prediction on the target domain data. To this end, we propose a few-shot transfer learning method, named learn-with-reference, that can learn knowledge from the existing dataset with reference to a small number of examples in the target domain so the model learns knowledge can well fit the underlying target domain data. The proposed learn-with-reference method can fit in the general supervised learning framework for saliency prediction and does not require any architecture changes to work with state-of-the-art saliency models. We use SALICON as the knowledge set and randomly select 1 or 5 samples from subset Inverted, Jumbled, and art from CAT2000. The experimental results show that the proposed learn-with-reference method efficiently transfers the knowledge learned from SALICON to the three target subsets. Furthermore, fine-tuning, as a transfer learning strategy, can work with the model trained with the proposed learn-with-reference method to improve the most of metrics. This suggests that the knowledge transferred by the proposed learn-with-reference method is aligned with the knowledge transferred by the fine-tuning, which is a common transfer strategy. The code and the experimental protocol are publicly available at \url{URL}.
%   More importantly, according to our experiments, we find that fine-tuning, as a transfer learning strategy, can further transfer  does not improve sAUC and the proposed learn-with-reference method boost

%The process of collecting human fixations is prohibitive for saliency prediction, especially in new domains where even lack the images.
%On the one hand, the target domain images could be different from the ones in the existing large-scale saliency dataset in terms of bottom-up stimulus and scene context. 
%On the other hand, according to the the biased competition theory, human attention is determined by the competition among objects in the visual field. 
%The competition mechanism can be seen as the knowledge that could be learned from the existing large-scale saliency dataset. 
%In this work, we propose a few-shot transfer learning method, named learn-with-reference, to adapt the source domain knowledge to the target domain. It only needs a small number of target domain examples and the existing saliency datasets as input. Moreover, the proposed learn-with-reference method does not require any architecture changes to work with state-of-the-art saliency models. We conduct comprehensive experiments to show that the proposed learn-with-reference method is efficient in the knowledge transfer to improve saliency prediction performance. More importantly, the experimental results suggest that the knowledge transferred by the proposed method is aligned with the one transferred by fine-tuning, which is a common transfer learning strategy. The code and the experimental protocol are publicly available at \url{https://anonymous.4open.science/r/99ea674c-9c72-46b9-b2df-f9f29f35fe35/}.

\end{abstract}
